Scalable Semi-Modular Inference with Variational Meta-Posteriors

The Cut posterior and related Semi-Modular Inference are Generalised Bayes methods for Modular Bayesian evidence combination. Analysis is broken up over modular sub-models of the joint posterior distribution. Model-misspecification in multi-modular models can be hard to fix by model elaboration alone and the Cut posterior and SMI offer a way round this. Information entering the analysis from misspecified modules is controlled by an influence parameter $\eta$ related to the learning rate. This paper contains two substantial new methods. First, we give variational methods for approximating the Cut and SMI posteriors which are adapted to the inferential goals of evidence combination. We parameterise a family of variational posteriors using a Normalising Flow for accurate approximation and end-to-end training. Secondly, we show that analysis of models with multiple cuts is feasible using a new Variational Meta-Posterior. This approximates a family of SMI posteriors indexed by $\eta$ using a single set of variational parameters.

==> notes.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%First attempt at cutting priors

The loss function for which $p_{cut}(\beta,\tau, \sigma|Y)\propto \exp(-l_{cut})p(\beta,\tau, \sigma)$ is a Gibbs posterior is
\begin{equation}\label{eq:HM_full_cut_loss}
  l_{cut}(Y; \beta,\tau, \sigma, \pi_0)=-\log(p(Y|\beta,\tau))-\log(p_{cut}(Y|\sigma))+\log(p(Y|\sigma))
\end{equation}
where $\pi_0(\sigma,\tau,\beta,\tilde\beta)=p(\sigma)p(\tau|\sigma)p(\beta|\tau)\tilde p(\tilde\beta)$ is the prior which we must specify as part of the loss as it appears in $p_{cut}(Y|\sigma)$ and $p(Y|\sigma)$ and changes as belief is updated.

\begin{proposition}
  The Cut-loss in \cref{eq:HM_full_cut_loss} is prequentially additive in the sense of \cite{Nicholls2022smi} for the belief update given by the Gibbs posterior and so (by Theorem~2.1 in that paper) the Cut posterior in \cref{eq:HM_full_cut_posterior} is an order coherent belief update.
\end{proposition}

\begin{proof} Let $Y^{(1)},Y^{(2)}$ be an arbitrary partition of $Y$. The loss $l_{cut}$ is prequentially additive if
  \begin{equation}\label{eq:HM_preq_add_defn}
    l_{cut}(Y; \beta,\tau, \sigma, \pi_0)=l_{cut}(Y^{(2)}; \beta,\tau, \sigma, \pi_1)+l_{cut}(Y^{(1)}; \beta,\tau, \sigma, \pi_0),
  \end{equation}
  where $\pi_1$ is the ``prior" for $\sigma,\tau,\beta,\tilde\beta$ after the first block of data $Y^{(1)}$ has arrived. By \cref{eq:HM_full_cut_posterior} this is $\pi_1(\sigma,\tau,\beta,\tilde\beta)=p_{cut}(\sigma,\tau,\beta,\tilde\beta|Y^{(1)})$.
  The LHS of \cref{eq:HM_preq_add_defn} is given in \cref{eq:HM_full_cut_loss}.
  The data are conditionally independent so $p(Y|\beta,\tau)=p(Y^{(2)}|\beta,\tau)p(Y^{(1)}|\beta,\tau)$, and the RHS is
  \begin{align*}
    l_{cut}(Y^{(2)}; \beta,\tau, \sigma, \pi_1)+l_{cut}(Y^{(1)}; \beta,\tau, \sigma, \pi_0)= &
    -\log(p(Y|\beta,\tau))                                                                                                                                                                                                                           \\
                                                                                             & -\log(p_{cut}(Y^{(2)}|\sigma,Y^{(1)}))+\log(p(Y^{(2)}|\sigma,Y^{(1)}))                                                                                \\
                                                                                             & -\log(p_{cut}(Y^{(1)}|\sigma))+\log(p(Y^{(1)}|\sigma))                                                                                                \\
    =                                                                                        & -\log(p(Y|\beta,\tau))                                                                                                                                \\
                                                                                             & -\log\left(\frac{p_{cut}(Y^{(2)},Y^{(1)}|\sigma)}{p_{cut}(Y^{(1)}|\sigma}\right)+\log\left(\frac{p(Y^{(2)},Y^{(1)}|\sigma)}{p(Y^{(1)}|\sigma)}\right) \\
                                                                                             & -\log(p_{cut}(Y^{(1)}|\sigma))+\log(p(Y^{(1)}|\sigma))                                                                                                \\
                                                                                             & =-\log(p(Y|\beta,\tau))-\log(p_{cut}(Y|\sigma))+\log(p(Y|\sigma))
  \end{align*}
  and we are done.
\end{proof}

We make some remarks on the proof and give some intuitiion for the particular objects which appear. In the expression for the prequentially additive loss, $p_{cut}(Y^{(2)}|\sigma,Y^{(1)})$ is conditioned on $Y^{(1)}$ because the prior $\pi_1(\tilde\beta|\sigma)$ used to form this marginal likelihood is
\[
  p_{cut}(\tilde\beta|\sigma,Y^{(1)})= \frac{1}{p_{cut}(Y^{(1)}|\sigma)}p(Y^{(1)}|\sigma,\tilde \beta)\tilde p(\tilde\beta).
\]
This is the prior in the imputation stage we get after a belief update from the original imputation stage prior. Similarly $p(Y^{(2)}|\sigma,Y^{(1)})$ is conditioned on $Y^{(1)}$ because the prior used to form this marginal likelihood is
\[
  p(\tau,\beta|\sigma,Y^{(1)})= \frac{p(Y^{(1)}|\sigma,\beta)}{p(Y^{(1)}|\sigma)}p(\beta|\tau)p(\tau|\sigma).
\]
This is the prior in the analysis stage we get after a belief update from the original imputation stage prior.

Now in brief for the first term on the second line of the loss expansion, $p_{cut}(Y^{(2)}|\sigma,Y^{(1)})=p_{cut}(Y^{(2)},Y^{(1)}|\sigma)/p_{cut}(Y^{(1)}|\sigma)$. This follows using conditional probability, since $p_{cut}(Y^{(2)}|\sigma,Y^{(1)})=p_{cut}(Y^{(2)},\sigma,Y^{(1)})/p_{cut}(\sigma,Y^{(1)})$.
More explicitly,
\begin{align*}
  p_{cut}(Y^{(2)}|\sigma,Y^{(1)})
   & =\int p(Y^{(2)}|\tilde\beta,\sigma,Y^{(1)}) p_{cut}(\tilde\beta|\sigma,Y^{(1)}) d\tilde\beta                                           \\
   & = \frac{1}{p_{cut}(Y^{(1)}|\sigma)}\int p(Y^{(2)}|\sigma,\tilde\beta) p(Y^{(1)}|\sigma,\tilde \beta)\tilde p(\tilde\beta) d\tilde\beta \\
   & =p_{cut}(Y|\sigma)/p_{cut}(Y^{(1)}|\sigma).
\end{align*}
In brief for the second term we have $p(Y^{(2)}|\sigma,Y^{(1)})=p(Y|\sigma)/p(Y^{(1)}|\sigma)$ by the same reasoning using the definition of conditional probability. More explicitly,
\begin{align*}
  p(Y^{(2)}|\sigma,Y^{(1)}) & =\int p(Y^{(2)}|\sigma,\beta)p(\tau,\beta|\sigma,Y^{(1)}) d\tau d\beta                                                 \\
                            & =\frac{1}{p(Y^{(1)}|\sigma)}\int p(Y^{(2)}|\sigma,\beta)p(Y^{(1)}|\tau,\beta,\sigma)p(\tau,\beta|\sigma) d\tau d\beta  \\
                            & =\frac{1}{p(Y^{(1)}|\sigma)}\int p(Y^{(2)}|\sigma,\beta)p(Y^{(1)}|\beta,\sigma)p(\beta|\tau)p(\tau|\sigma)d\tau d\beta \\
                            & =\frac{p(Y|\sigma)}{p(Y^{(1)}|\sigma)}
\end{align*}

.
.
.

When we wish to drop a prior factor (such as $p(\beta|\tau)$ in the present example) in the imputation stage, we cannot simply remove the prior for the random variable ($\beta$ here). Because it must have some prior distribution for subsequent conditioning, the imputation and analysis posteriors can differ by replacement of a prior factor, whilst they can differ by replacement or removal of a likelihood factor.
In our example we would like to stop the misspecified $p(\beta |\tau)$ prior from distorting the estimation of $\sigma$.
When we remove this prior factor for $\beta$ we have to give a replacement prior for $\beta$ for use in the imputation stage. Call this prior $\tilde p(\tilde\beta)$. The random variables $\beta$ and $\tilde\beta$ have different distributions so we distinguish them. We have now to choose this imputation prior $\tilde p$. In our example we make $\tilde p(\tilde\beta)\propto 1$.

we must have different random variables in the imputation stage (in $p_{cut}(\sigma,\tilde\beta|Y)$ where $\tilde\beta$ has prior density $\tilde p(\cdot)$) and the analysis stage (in $p(\tau,\beta|Y,\sigma)$ where $\tilde\beta$ has prior density $p(\beta|\tau)$). In previous work it has often been implicit that the prior used for replacement was the uniform distribution as that is what you get if you replace ``$p(\beta|\tau)$" with ``1".

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Material from the Meta-post section - includes GN stuff on
%multiple modules and CC stuff setting up MP's.

Consider a multi-modular model with $M$ modules indexed $\mathcal{M}=\{1,...,M\}$. In order to fix ideas we consider the following setup. Let $\mathcal{D}=(D_1,...,D_M)$ with $D_m,\ m\in \mathcal{M}$ be the data in module $m$ and let $\Psi=(\psi_1,...,\psi_A)$ be the collection of all parameters in the model. For $m\in \mathcal{M}$ let $i_m\subseteq \{1,...,A\}$ be the subset of indices for parameters entering the generative model for data $D_m$ and no other module (intrinsic parameters) and  let $e_{m}\subseteq \{1,...,A\}$ be the indices of parameters which module $m$ shares with other modules (extrinsic).
Let $p_m(D_m \mid \psi_{i_m},\psi_{e_m})$ be the observation model for module $m$ and let $p_m(\psi_{i_m} \mid \psi_{e_m})$ be the prior for the intrinsic parameters of module $m$ given its extrinsic parameters.
Let $E=\cup_m e_m$ be the set of all extrinsic parameter indices. The joint Bayes posterior can be written
\begin{equation}
  p(\Psi|\mathcal{D}) = p(\psi_{E})\prod_{m\in \mathcal{M}} p_m(D_m \mid \psi_{i_m},\psi_{e_m})\, p_m(\psi_{i_m} \mid \psi_{e_m}).
\end{equation}
Suppose a subset of modules $\mathcal{C}\subset \mathcal{M},\ \mathcal{C}=\{c_1,...,c_N\}$ have been identified as possibly misspecified and we wish to cut or modulate their influence on other modules.
Let $H=[0,1]^N$ be the space of influence parameters $\eta\in H,\ \eta=(\eta_1,...,\eta_N)$. The joint \acrshort{smi} posterior is
\begin{align}
  p_{\text{smi},\eta}(\Psi|\mathcal{D}) & \propto p(\psi_{E})\prod_{b\in \mathcal{C}}
  p_b(D_b\mid\tilde\psi_{i_b},\psi_{e_b})^{\eta_b}\, p_b(\tilde\psi_{i_b} \mid \psi_{e_b})
  \\
                                        & \qquad\times\quad
  \prod_{m\in \mathcal{M}\setminus \mathcal{C}} p_m(D_m \mid \psi_{i_m},\psi_{e_m})\, p_m(\psi_{i_m} \mid \psi_{e_m})
  \\
                                        & \qquad\times\quad
  \prod_{c\in \mathcal{C}} p_c(\psi_{i_c} \mid D_c, \psi_{e_c})                       \\
                                        & =p_{\text{pow},\eta}()
\end{align}
This is still
For a given probabilistic model defined in a multi-modular setting $p(\Psi, \mathcal{D})$, with parameters $\Psi$, data $\mathcal{D}$ and $M$ cuts, \acrlong*{smi} defines a \emph{family} of posterior distributions $\mathcal{P}_{smi}=\{p_{ \text{smi}, \eta}(\Psi \mid \mathcal{D}) \;,\;\eta \in H \}$, characterised by $\eta \in H$, the \emph{rates of feedback} between modules, taking values in $H=[0,1]^M$.
The \acrshort*{smi} posterior at $\Psi$ is a continuous and differentiable function of $\eta$, so we would expect that $\mathcal{P}_{smi}$ is a connected set.

Given a variational family $\mathcal{Q}=\{q_{\lambda}(\Psi), \lambda \in \Lambda\}$ (with variational parameters $\lambda$) there is a subset of elements that best approximate the elements in the \acrshort*{smi} family, $\mathcal{Q}_{smi} = \{ q: \argmin_{q \in \mathcal{Q}} D(q{\,{\,\|\,}\,} p) , p \in \mathcal{P}_{smi} \} \subset \mathcal{Q}$.
Let us denote the associated set of variational parameters as $\Lambda_{smi}=\{ \lambda : q_{\lambda} \in \mathcal{Q}_{smi} \} \subset \Lambda$.

In practice, we are interested in choosing the best element of $p_{ \text{smi}, \eta} \in \mathcal{P}_{smi}$ for some performance score.
By using the variational approximation described in \cref{sec:vsmi}, we aim to solve the proxy problem of finding the best $q_{\lambda} \in \mathcal{Q}_{smi}$.

The correspondence between $\eta$ and the variational parameters $\lambda$ that best approximate $p_{ \text{smi}, \eta}$ is not one-to-one in general.
Variational families with highly flexible distributions may contain multiple elements which solve the minimisation problem.
Nevertheless, if the variational family $\mathcal{Q}$ is smooth with respect to the variational parameters, we would expect that $\Lambda_{smi}$ is composed as the union of connected sets.

When $\Lambda_{smi}$ is a single connected set, the optimal variational parameters for a given $\eta$ provides useful information for the optimisation of a neighbour $\eta+\epsilon$.
If $\Lambda_{smi}$ is composed by the union of multiple sets, independent optimisation via \acrshort*{sgd} for different values of $\eta$ may output $\hat\lambda$'s in different regions, which is not convenient for our purpose of exploration along $\eta\in H$.
This leads us to consider optimisation strategies that are able to a) favour \emph{continuity} in $\hat\Lambda_{smi}$ as a function of $\eta$, and b) share information between the optimisation of all $\eta \in H$.

We propose a method to learn a connected set of parameters $\hat\Lambda_{smi}$ by learning a continuous mapping,

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This is equivalent to minimize the negative \acrshort*{elbo},
\begin{align}
  \text{ELBO}^{(\eta-\text{smi})} = \E_{(\varphi, \theta, \tilde\theta) \sim q(\varphi, \theta, \tilde\theta)}[ & \log p(Z \mid \varphi) + \eta \log p(Y \mid \varphi, \tilde\theta) + \log p(\varphi, \tilde\theta) \nonumber \\
                                                                                                                & + \log p(Y \mid \varphi, \theta) + \log p(\varphi, \theta) - \log p(Y, \varphi) \nonumber                    \\
                                                                                                                & - \log q(\varphi, \theta, \tilde\theta) ]
\end{align}

The gradients of $\text{ELBO}^{(\eta-\text{smi})}$ w.r.t. our variational parameters are:
\begin{align}
  \nabla_{\lambda_1} \text{ELBO}^{(\eta-\text{smi})} = \E_{\epsilon \sim p(\epsilon)}[ & \nabla_{\varphi} \left\{ \log p(Z \mid \varphi) + \eta \log p(Y \mid \varphi, \tilde\theta) + \log p(\varphi) \right\} \nabla_{\lambda_1} \{ \varphi \} \nonumber    \\
                                                                                       & + \nabla_{\varphi} \left\{ \log p(Y \mid \varphi, \theta) + \log p(\varphi) + \log p(Y, \varphi) \right\} \nabla_{\lambda_1} \{ \varphi \} \nonumber                 \\
                                                                                       & + \nabla_{\lambda_1} \log \left| J_{T_1} \right| ] \label{eq:grad_elbo_l1_smi_naive}                                                                                 \\
  \nabla_{\lambda_2} \text{ELBO}^{(\eta-\text{smi})} = \E_{\epsilon \sim p(\epsilon)}[ & \nabla_{\theta} \left\{ \log p(Y \mid \varphi, \theta) + \log p(\theta \mid \varphi) \right\} \nabla_{\lambda_2} \{ \theta \} \nonumber                              \\
                                                                                       & + \nabla_{\lambda_2} \log \left| J_{T_2} \right| ] \label{eq:grad_elbo_l2_smi}                                                                                       \\
  \nabla_{\lambda_3} \text{ELBO}^{(\eta-\text{smi})} = \E_{\epsilon \sim p(\epsilon)}[ & \nabla_{\tilde\theta} \left\{ \eta \log p(Y \mid \varphi, \tilde\theta) + \log p(\tilde\theta \mid \varphi) \right\} \nabla_{\lambda_3} \{ \tilde\theta \} \nonumber \\
                                                                                       & + \nabla_{\lambda_3} \log \left| J_{T_3} \right| ] \label{eq:grad_elbo_l3_smi}
\end{align}

By analysing these gradients, we notice that this naive approximation is not the best way to approximate the \acrshort*{smi} posterior.
When $\eta=1$, the $p_{\eta-smi}(\varphi,\theta)$ is equivalent to the conventional fully-Bayesian posterior.
Therefore it is desirable to obtain a match between \cref{eq:grad_elbo_l1_full,eq:grad_elbo_l1_smi_naive}, and also have symmetry between \cref{eq:grad_elbo_l2_full,eq:grad_elbo_l2_smi,eq:grad_elbo_l3_smi} \todo{why?}.
Nevertheless, the second line in \cref{eq:grad_elbo_l1_smi_naive} is inconvenient, creating bias in the estimation of the desired gradient.
Moreover, the term $\nabla_{\varphi} \log p(Y, \varphi) \nabla_{\lambda_1} \{ \varphi \}$, is intractable and only can be evaluated for very simple models.

We would like to remove the whole middle line from the gradient in \cref{eq:grad_elbo_l1_smi_naive} in order to obtain an equivalent approximation between \acrshort*{smi} posterior with $\eta=1$ and conventional full posterior.

To understand the role of this term in the optimization process, consider the following decomposition of our target \acrshort*{kl} divergerce (derivation in the supplement),
\begin{align*}
  \kl{ q(\varphi, \theta, \tilde\theta) }{ p_{\eta-smi}(\varphi, \theta, \tilde\theta \mid Z, Y) } & =                                                                                                             \\
  \kl{ q(\varphi, \tilde\theta) }{ p_{\eta-pow}(\varphi, \tilde\theta \mid Z, Y) }                 & + \E_{\varphi \sim q(\varphi)}\left[ \kl{ q(\theta \mid \varphi) }{ p(\tilde\theta \mid Y, \varphi) } \right]
\end{align*}

We see that $q(\varphi)$ plays in two positions here: on one hand, approximates the power posterior jointly with $\tilde\theta$; and on the other, it helps to improve the approximation to the conditional posterior $p(\theta \mid Y, \varphi)$
Removing the middle line in \cref{eq:grad_elbo_l1_smi_naive} is equivalent to removing the second "objective" for $q(\varphi)$.

Removing the problematic term is also justified intuitively in the case of $\eta=0$, where $p_{\eta-smi}(\varphi,\theta)$ is equivalent to the cut posterior.
In this case, we don't want $q(\eta)$ to receive any feedback from the $Y$ module.
Removing this term effectively accomplishes that for our variational approximation.

We propose a loss function $\mathcal{L}^{(\eta-\text{smi})}$ to approximate the \acrshort*{smi} posterior adequately,
\begin{align} \label{eq:vsmi_loss}
  \mathcal{L}^{(\eta-\text{smi})} = -\E_{(\varphi, \theta, \tilde\theta) \sim q(\varphi, \theta, \tilde\theta)}[ & \log p_{\eta-pow}(Z, Y, \varphi, \tilde\theta) \nonumber   \\
                                                                                                                 & + \log p(Z, Y, \cancel{\nabla}(\varphi), \theta) \nonumber \\
                                                                                                                 & - \log q(\varphi, \theta, \tilde\theta) ]
\end{align}
where $\cancel{\nabla}(\cdot)$ denotes the \texttt{stop\_gradient} operator, and $p_{\eta-pow}(Z, Y, \varphi, \tilde\theta) = p(Z\mid\varphi)p(Y \mid \varphi, \tilde\theta)^{\eta}p(\varphi, \tilde\theta)$


The gradients of $-\mathcal{L}^{(\eta-\text{smi})}$ are,
\begin{align}
  -\nabla_{\lambda_1} \mathcal{L}^{(\eta-\text{smi})} = \E_{\epsilon \sim p(\epsilon)}[ & \nabla_{\varphi} \left\{ \log p(Z \mid \varphi) + \eta \log p(Y \mid \varphi, \tilde\theta) + \log p(\varphi) \right\} \nabla_{\lambda_1} \{ \varphi \} \nonumber    \\
                                                                                        & + \nabla_{\lambda_1} \log \left| J_{T_1} \right| ] \label{eq:grad_smi_loss_l1}                                                                                       \\
  -\nabla_{\lambda_2} \mathcal{L}^{(\eta-\text{smi})} = \E_{\epsilon \sim p(\epsilon)}[ & \nabla_{\theta} \left\{ \log p(Y \mid \varphi, \theta) + \log p(\theta \mid \varphi) \right\} \nabla_{\lambda_2} \{ \theta \} \nonumber                              \\
                                                                                        & + \nabla_{\lambda_2} \log \left| J_{T_2} \right| ] \label{eq:grad_smi_loss_l2}                                                                                       \\
  -\nabla_{\lambda_3} \mathcal{L}^{(\eta-\text{smi})} = \E_{\epsilon \sim p(\epsilon)}[ & \nabla_{\tilde\theta} \left\{ \eta \log p(Y \mid \varphi, \tilde\theta) + \log p(\tilde\theta \mid \varphi) \right\} \nabla_{\lambda_3} \{ \tilde\theta \} \nonumber \\
                                                                                        & + \nabla_{\lambda_3} \log \left| J_{T_3} \right| ] \label{eq:grad_smi_loss_l3}
\end{align}

The \texttt{stop\_gradient} operator has the effect of removing a summand that would otherwise appear inside the expectation of \cref{eq:grad_smi_loss_l1}, namely
\begin{equation*}
  \nabla_{\varphi} \left\{ \log p(Z \mid \varphi) + \log p(Y \mid \varphi, \theta) + \log p(\varphi) \right\} \nabla_{\lambda_1} \{ \varphi \}
\end{equation*}

In the case $\eta=1$, we obtain a match between the gradients of \cref{eq:grad_elbo_l1_full,eq:grad_smi_loss_l1}, and symmetry between \cref{eq:grad_elbo_l2_full,eq:grad_smi_loss_l2,eq:grad_smi_loss_l3}, effectively approximating the full posterior.

In the case $\eta=0$, the gradient in \cref{eq:grad_smi_loss_l1} is not influenced by $Y$ or $\theta$, it only depends on elements from the first module.
The loss in this case can be interpreted as a two-stage optimisation procedure:

\begin{enumerate}
  \item Learn $q_{\lambda_1}(\varphi)$ through conventional variational inference over the module $Z$,
        \begin{equation*}
          \lambda_1^* = \argmin_{\lambda_1} \kl{ q_{\lambda_1}(\varphi) }{ p(\varphi \mid Z) }
        \end{equation*}
  \item Learn the conditional variational posterior $q_{\lambda_2}(\theta \mid \varphi)$ in a similar way to variational inference over the full model, but preserving the marginal posterior of $\varphi$ obtained from stage 1.
        \begin{equation*}
          \lambda_2^* = \argmin_{\lambda_2} \kl{ q_{\lambda_1^*,\lambda_2}(\varphi,\theta) }{ p(\varphi,\theta \mid Z, Y) }
        \end{equation*}
\end{enumerate}

This two-stage optimization procedure to target the variational \acrshort*{smi} posterior is similar to the interpretation of the cut posterior as a constrained optimization problem, as proposed by \cite{Yu2021variationalcut}.

The two-stage interpretation of our loss is also valid for other values $\eta \in (0,1)$, but the first stage would approximate the power posterior in that case.
